Joint Wireless and Edge Computing Resource Management with Dynamic Network Slice Selection

Network slicing is a promising approach for enabling low latency computation offloading in edge computing systems. In this paper, we consider an edge computing system under network slicing in which the wireless devices generate latency sensitive computational tasks. We address the problem of joint dynamic assignment of computational tasks to slices, management of radio resources across slices and management of radio and computing resources within slices. We formulate the Joint Slice Selection and Edge Resource Management(JSS-ERM) problem as a mixed-integer problem with the objective to minimize the completion time of computational tasks. We show that the JSS-ERM problem is NP-hard and develop an approximation algorithm with bounded approximation ratio based on a game theoretic treatment of the problem. We provide extensive simulation results to show that network slicing can improve the system performance compared to no slicing and that the proposed solution can achieve significant gains compared to the equal slicing policy. Our results also show that the computational complexity of the proposed algorithm is approximately linear in the number of devices.

==> network_level_complete_info.tex <==
\section{Existence of Stackelberg Equilibria}
\label{sec::network_level_complete_information}
In this section we analyze the interaction between the network operator and the slices. 
We use backward induction to prove the existence of equilibria, i.e., we first consider problem (\ref{eq::slices_BR})-(\ref{cons::slices_BR}) solved by the slices, and then we consider problem (\ref{eq::operator_BR_complete_information})-(\ref{cons::operator_BR_complete_information}) solved by the \ac{SRO}.

\subsection{\rev{Equilibrium Allocation Policy Within Slices}}
\rev{In what follows we provide closed form expressions for the equilibrium allocation policies of slices.}

\begin{theorem}\label{theo::opt_sharing_policy_slices}
 \rev{Let $\varpolicy_\varbandwidthslicecoef$ and $\vardecisionsvector$ be an inter-slice radio allocation policy and an offloading decision vector determined by the \ac{SRO}, respectively.}
 The equilibrium allocation policy $(\varpolicy_\varuplinkratecoef^{\varAP,\varslice,*},\varpolicy_\varcomppowercoef^{\varslice,*})$ of slice $\varslice$ sets the \rev{intra-slice radio} provisioning coefficients for every WD $\varplayer \!\in\! \varoffloaders_{(\varAP,\varslice)}(\vardecisionsvector)$, $\forall \varAP \!\in\! \varAPsset$, and computing power provisioning coefficients for every WD $\varplayer \!\in\! \varoffloaders_{(\varcloud,\varslice)}(\vardecisionsvector)$, $\forall \varcloud \!\in\! \varcloudsset$ according to
 \begin{eqnarray}\label{eq::optimal_slice-resource_coef}
  \varuplinkratecoef_{\varplayer,\varAP}^{\varslice,*} \!=\! \frac{\sqrt{\vardatasize_\varplayer/\varphywirelessrate_{\varplayer,\varAP}}}{\!\!\!\!\sum \limits_{\varoplayer \in \varoffloaders_{(\varAP,\varslice)}(\vardecisionsvector)}\!\!\!\!\!\!\!\!\!\!\sqrt{\vardatasize_\varoplayer/\varphywirelessrate_{\varoplayer,\varAP}}} \text{ and } \varcomppowercoef_{\varplayer,\varcloud}^{\varslice,*} \!=\! \frac{\rev{\sqrt{\vartaskcomplexity_\varplayer/\vardeviceslicecoef_{\varplayer,\varslice}}}}{\!\!\!\!\sum \limits_{\varoplayer \in \varoffloaders_{(\varcloud,\varslice)}(\vardecisionsvector)}\!\!\!\!\!\!\!\!\!\!\sqrt{\rev{\vartaskcomplexity_\varoplayer/\vardeviceslicecoef_{\varoplayer,\varslice}}}},
 \end{eqnarray} 
respectively.
\end{theorem}
\begin{proof} 
\rev{From the definition~(\ref{eq::cost_per_slice}) of the cost per slice it is easy to see that for given $\vardecisionsvector$ problem (\ref{eq::slices_BR})-(\ref{cons::slices_BR}) solved by slice $\varslice \in \varslicesset$ is equivalent to problem (\ref{eq::objective_slices})-(\ref{eq::slices_both_constraint}) for $\mathcal{F} = \varAPsset \cup \varcloudsset$ and $\mathcal{S} = \{\varslice\}$. Furthermore, by suitably defining variables $x_{i,f}^s$ and constants $A_{i,f}^s$ in~(\ref{eq::optimal_coef_slices}), we can obtain expressions for coefficients $\varuplinkratecoef_{\varplayer,\varAP}^{\varslice,*}$ and $\varcomppowercoef_{\varplayer,\varcloud}^{\varslice,*}$ in~(\ref{eq::optimal_slice-resource_coef}), which proves the theorem.}
\end{proof}
 Next, for notational convenience let us define the set of resources $\varactiveresourcesset = \{\{\varAPsset \times \varslicesset\} \cup \{\varcloudsset \times \varslicesset\} \cup \varactiveplayersset\}$ and let us introduce the following shorthand notation
\begin{eqnarray}\label{eq::weights}\nonumber
  &\hspace{-0.2cm}\varcongestionweight_{\varplayer,(\varAP,\varslice)} \triangleq \sqrt{\vardatasize_\varplayer/\varphywirelessrate_{\varplayer,\varAP}}, \text{        }\varcongestionweight_{\varplayer,(\varcloud,\varslice)}\triangleq \sqrt{\rev{\vartaskcomplexity_\varplayer/\vardeviceslicecoef_{\varplayer,\varslice}}}, \text{        }\varcongestionweight_{\varplayer,\varplayer} \triangleq \sqrt{\vartaskcomplexity_\varplayer},\\
%\end{equation}
%\begin{equation}\label{eq::congestions}
   &\varcongestionweight_{\varresource}(\vardecisionsvector) \triangleq \sum \nolimits_{\varoplayer \in \varoffloaders_{\varresource}(\vardecisionsvector)}\varcongestionweight_{\varoplayer,\varresource}, \forall \varresource \in \varresourcesset.
\end{eqnarray}

By substituting (\ref{eq::optimal_slice-resource_coef}) into (\ref{eq::uplink_rate}) and (\ref{eq::cloud_to_user_power}) and by using the notation introduced in (\ref{eq::weights}), we can express the cost (\ref{eq::user_i_cost}) of WD $\varplayer$ under the collection $(\varpolicy_\varuplinkratecoef^{\varAP,*},\varpolicy_\varcomppowercoef^{\varcloud,*})$ of equilibrium allocation policies of slices as 
\begin{equation}\label{eq::WD_cost_under_opt_slices_any_operator}
    \Tilde{\varcost}_\varplayer(\vardecisionsvector,\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*) = \sum \nolimits_{\varresource \in \varresourcesset_{\vardecision_\varplayer}} m_\varresource \varcongestionweight_{\varplayer,\varresource}\varcongestionweight_\varresource(\vardecisionsvector),
\end{equation}
where $\varresourcesset_{\vardecision_\varplayer}$ is the set of resources that WD $\varplayer$ uses for performing its task in strategy profile $\vardecisionsvector$ (i.e., $\varresourcesset_{\vardecision_\varplayer} \subset \varresourcesset$) and $m_{(\varAP,\varslice)} = 1/\varbandwidthslicecoef_\varAP^\varslice$, $m_{(\varcloud,\varslice)} = 1/\varcomppower_\varcloud^\varslice$ and $m_{\varplayer} = 1/\varcomppower_\varplayer^\varlocal$.

Finally, by summing the expressions (\ref{eq::WD_cost_under_opt_slices_any_operator}) over all WDs $\varplayer \in \varactiveplayersset$ and by reordering the summations we can express the system cost (\ref{eq::system_cost}) under the collection $(\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$ of equilibrium allocation policies of slices as 
\begin{eqnarray}\label{eq::system_cost_under_optimal_slices_sumations_organised}
    &\hspace{-0.6cm}\Tilde{\varcost}(\vardecisionsvector,\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*) = \sum \nolimits_{\varresource \in \varactiveresourcesset} m_\varresource\varcongestionweight_\varresource^2(\vardecisionsvector).
\end{eqnarray}

\subsection{\rev{Equilibrium Solution Across Slices}}
\label{sec::eq_sol_across_slices}
\rev{We continue with considering the problem (\ref{eq::operator_BR_complete_information})-(\ref{cons::operator_BR_complete_information}) solved by the \ac{SRO}.}

 \subsection{\rev{Equilibrium Allocation Policy Across Slices}}
 \rev{We continue with providing closed form expressions for the equilibrium allocation policy of the \ac{SRO}.}
\begin{theorem}\label{theo::opt_sharing_policy_operator}
\rev{Consider that each slice $\varslice \in \varslicesset$ allocates bandwidth and computing resources according to the equilibrium policy $(\varpolicy_\varuplinkratecoef^{\varslice,*},\varpolicy_\varcomppowercoef^{\varslice,*})$, which sets intra-slice radio and computing power provisioning coefficients according to (\ref{eq::optimal_slice-resource_coef}) and that offloading decisions of WDs are determined according to some strategy profile $\vardecisionsvector$}. Then, the equilibrium allocation policy $\varpolicy_\varbandwidthcoef^*$ of the \ac{SRO} sets the \rev{inter-slice radio} provisioning coefficients for every slice $\varslice \in \varslicesset$ according to
 \begin{eqnarray}\label{eq::optimal_operator_slice_coef}
  \varbandwidthcoef_{\varAP}^{\varslice,*} \!=\! \frac{\varcongestionweight_{(\varAP,\varslice)}(\vardecisionsvector)}{\sum \nolimits_{\varoslice \in \varslicesset} \varcongestionweight_{(\varAP,\varoslice)}(\vardecisionsvector)}.
 \end{eqnarray} 
\end{theorem}
\begin{proof}
\rev{Observe that the system cost function (\ref{eq::system_cost_under_optimal_slices_sumations_organised}) can be expressed in the form of the objective function (\ref{eq::SRO_objective}), and thus problem (\ref{eq::operator_BR_complete_information})-(\ref{cons::operator_BR_complete_information}) of the \ac{SRO} has the same form as problem (\ref{eq::SRO_objective})-(\ref{eq::SRO_both_constraint}). Therefore, by adequately defining variables $b_f^s$ and constants $A_{i,f}^s$ in~(\ref{eq::optimal_coef_SRO}), we can obtain expression~(\ref{eq::optimal_operator_slice_coef}) for coefficients $\varbandwidthslicecoef_{\varAP}^{\varslice,*}$, which proves the theorem.}
%Similarly as in the case of slices' problems, we observe that the problem (\ref{eq::operator_BR_complete_information})-(\ref{cons::operator_BR_complete_information}) of the \ac{SRO} has the same form as problem (\ref{eq::general_objective})-(\ref{eq::constraint_sum_of_variables}) as the decision variables $\varbandwidthslicecoef_\varAP^\varslice$ appear in the expressions of the form $\frac{A^2}{\varbandwidthslicecoef_{\varAP}^{\varslice}}$, where $A^2$ is a correspondingly defined constant. Therefore, by following the proof of Lemma~\ref{lemm::general_closed_form_expressions} we can obtain the expression~(\ref{eq::optimal_operator_slice_coef}) for coefficients $\varbandwidthslicecoef_{\varAP}^{\varslice,*}$, which proves the theorem.
\end{proof}
%Finally, based on Theorem~\ref{theo::opt_sharing_policy_slices} and Theorem~\ref{theo::opt_sharing_policy_operator} we can formulate the following result.
%\begin{corollary}\label{cor::SPE_existence_in_NL-BAG}
%Let $\vardecisionsvector$ be a strategy profile of WDs. Then $(\vardecisionsvector,\varpolicy_\varbandwidthcoef^*,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$ is an SPE of \ac{NL-BAG}.
%\end{corollary}




==> network_level_incomplete_info.tex <==
\section{Incomplete Information Operator}
\label{sec::network_level_complete_information}
\todo[inline]{Proposition 1 (each slice has it's own set of users -> cost is convex)
Corollary: Stochastic approximation could be used for optimizing slice bandwidth allocation.
In general the cost is not convex, hence we propose to use Bayesian optimization}

==> slice_level.tex <==
\subsection{\rev{Equilibrium of Offloading Decisions}}
\label{sec::slice_level}
\rev{In the following we provide an approximation algorithm for computing an equilibrium vector $\vardecisionsvector^*$ of offloading decisions. }
\todo[inline]{@Sladjana continue from here}
First, using the notation introduced in (\ref{eq::weights}) we define the cost of sharing resource $\varresource \!\in\! \varresourcesset$ in strategy profile $\vardecisionsvector$ as
\begin{equation}\label{eq::AP_s_cost}
    \varresourcecost_{(\varAP,\varslice)}(\vardecisionsvector,\varpolicy_\varbandwidthcoef) \triangleq m_{(\varAP,\varslice)}\varcongestionweight_{(\varAP,\varslice)}(\vardecisionsvector),
\end{equation}
\begin{equation}\label{eq::cloud_s_cost_and_local_cost}
    \varresourcecost_{(\varAP,\varcloud)}(\vardecisionsvector) \triangleq m_{(\varcloud,\varslice)}\varcongestionweight_{(\varcloud,\varslice)}(\vardecisionsvector), \text{        }\varresourcecost_{\varplayer}(\vardecisionsvector) \triangleq m_\varplayer\varcongestionweight_{\varplayer}(\vardecisionsvector).
\end{equation}
\begin{comment}
\begin{equation}\label{eq::AP_s_cost}
    \varresourcecost_{(\varAP,\varslice)}(\vardecisionsvector,\varpolicy_\varbandwidthcoef) \triangleq \varcongestionweight_{(\varAP,\varslice)}(\vardecisionsvector)/\varbandwidthcoef_\varAP^\varslice,
\end{equation}
\begin{equation}\label{eq::cloud_s_cost_and_local_cost}
    \varresourcecost_{(\varAP,\varcloud)}(\vardecisionsvector) \triangleq \varcongestionweight_{(\varcloud,\varslice)}(\vardecisionsvector)/\varcomppower_\varcloud^\varslice, \text{        }\varresourcecost_{\varplayer}(\vardecisionsvector) \triangleq \varcongestionweight_{\varplayer}(\vardecisionsvector)/\varcomppower_\varplayer^\varlocal.
\end{equation}
\end{comment}

We are now ready to formulate our next result concerning the strategic interactions between WDs under the collection $(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$ of policies.
\begin{theorem}
Consider that each slice $\varslice \in \varslicesset$ uses resource allocation policies $(\varpolicy_{\varuplinkratecoef}^{\varslice,*},\varpolicy_{\varcomppowercoef}^{\varslice,*})$, which set the \rev{intra-slice radio} $\varuplinkratecoef_{\varplayer,\varAP}^{\varslice,*}$ and the computing power $\varcomppowercoef_{\varplayer,\varcloud}^{\varslice,*}$ provisioning coefficients according to (\ref{eq::optimal_slice-resource_coef}), and that the operator uses some allocation policy $\varpolicy_\varbandwidthcoef$ for setting \rev{inter-slice radio} provisioning coefficients $\varbandwidthslicecoef_\varAP^\varslice$. Then, the strategic interactions of WDs can be modeled as a congestion game with resource-dependent weights $\varcongestionweight_{\varplayer,\varresource}$, $\varplayer \in \varactiveplayersset, \varresource \in \varactiveresourcesset$, and the cost of WD $\varplayer$ in the resulting game is given by
\begin{equation}\label{eq::congestion_game_device_cost}
\Tilde{\varcost}_{\varplayer}(\vardecisionsvector,\varpolicy_\varbandwidthcoef) = \!\!\!\!\!\!\sum_{\varresource \in \varresourcesset_{\vardecision_\varplayer} \cap \{\varAPsset \times \varslicesset\}} \!\!\!\!\!\!\!\!\!\!\!\!\!\varcongestionweight_{\varplayer,\varresource}\varresourcecost_\varresource(\vardecisionsvector,\varpolicy_\varbandwidthcoef) + \!\!\!\!\!\!\sum_{\varresource \in \varresourcesset_{\vardecision_\varplayer} \cap \{\{\varcloudsset \times \varslicesset\} \cup \{\varplayer\}\}}\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\! \varcongestionweight_{\varplayer,\varresource}\varresourcecost_\varresource(\vardecisionsvector).\!\!
\end{equation}
\end{theorem}
\begin{proof}
By using (\ref{eq::AP_s_cost}) and (\ref{eq::cloud_s_cost_and_local_cost}), we can express the cost (\ref{eq::WD_cost_under_opt_slices_any_operator}) of WD $\varplayer$ as (\ref{eq::congestion_game_device_cost}). Observe that $\varcongestionweight_{\varplayer,\varresource}$ can be interpreted as the weight that WD $\varplayer$ contributes to the congestion when using resource $\varresource$ and thus $\varcongestionweight_{\varresource}(\vardecisionsvector)$ can be interpreted as the total congestion on resource $\varresource$ in strategy profile $\vardecisionsvector$. Hence, the cost (\ref{eq::congestion_game_device_cost}) of WD $\varplayer$ in strategy profile $\vardecisionsvector$ depends on its own resource-dependent weights $\varcongestionweight_{\varplayer,\varresource}$ and on the total congestion $\varcongestionweight_{\varresource}(\vardecisionsvector)$ on the resources it uses, and thus it follows from~\cite{harks2011characterizing} that the resulting game played by WDs can be modeled as a congestion game with resource dependent weights, which proves the result.
\end{proof}
We refer to the resulting strategic game as $\varthegame(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*) = <\varactiveplayersset,(\varactivedecisionsset_\varplayer)_{\varplayer \in \varactiveplayersset},(\Tilde{\varcost}_\varplayer(\varpolicy_\varbandwidthcoef))_{\varplayer \in \varactiveplayersset}>$, in which the players are WDs with the objective to minimize their costs given by (\ref{eq::congestion_game_device_cost}). 
Observe that the game $\varthegame(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$ is the \ac{SL-COG} expressed in strategic form, thus to show that the \ac{SL-COG} has an SPE it is sufficient to show that the game $\varthegame(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$ has a pure strategy Nash equilibrium, defined as follows. 

\begin{definition}{({\bf BR and Pure NE})}
For a strategic game $\varthegame = <\varactiveplayersset,(\varactivedecisionsset_\varplayer)_{\varplayer \in \varactiveplayersset},(\Tilde{\varcost}_\varplayer)_{\varplayer \in \varactiveplayersset}>$ we define a better reply of player $\varplayer$ in a strategy profile $\vardecisionsvector = (\vardecision_\varplayer,\vardecision_{-\varplayer})$ as a strategy $\vardecision{}^{\prime}_\varplayer$ such that $\Tilde{\varcost}_{\varplayer}(\vardecision{}^{\prime}_\varplayer,\vardecision_{-\varplayer}) \leq \Tilde{\varcost}_{\varplayer}(\vardecision_\varplayer,\vardecision_{-\varplayer})$, and a best reply (BR) of player $\varplayer$ as a strategy $\vardecision{}^{*}_\varplayer$ such that $\Tilde{\varcost}_{\varplayer}(\vardecision{}^{*}_\varplayer,\vardecision_{-\varplayer}) \leq \Tilde{\varcost}_{\varplayer}(\vardecision_\varplayer,\vardecision_{-\varplayer}), \forall \vardecision_\varplayer \in \varactivedecisionsset_\varplayer$.

A pure strategy Nash equilibrium (NE) of the game $\varthegame$ is a strategy profile $\vardecisionsvector{}^{*}$ in which all players play their BRs to each others' strategies, i.e,
$$\bar{\varcost}_{\varplayer}(\vardecision{}^{*}_\varplayer,\vardecision{}^{*}_{-\varplayer} )\leq \Tilde{\varcost}_{\varplayer}(\vardecision_\varplayer,\vardecision{}^{*}_{-\varplayer}), \forall \vardecision_{\varplayer} \in \varactivedecisionsset_\varplayer, \forall \varplayer \in \varactiveplayersset.$$
\end{definition}

Thus, in what follows we focus on the existence of pure NE for $\varthegame(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$, and we start with recalling the definition of an exact potential function from~\cite{monderer1996potential}.
\begin{definition}
A function $\varpotentialfunction: \times_\varplayer (\varactivedecisionsset_\varplayer) \rightarrow \mathbb{R}$ is an exact potential for a finite strategic game $\varthegame = <\varactiveplayersset,(\varactivedecisionsset_\varplayer)_{\varplayer \in \varactiveplayersset},(\Tilde{\varcost}_\varplayer)_{\varplayer \in \varactiveplayersset}>$ if for an arbitrary strategy profile $(\vardecision_\varplayer,\vardecision_{-\varplayer})$ and for any better reply $\vardecision{}^\prime_\varplayer$ the following holds
\begin{equation}\label{eq::potential_function_def}
\Tilde{\varcost}\varplayer(\vardecision{}^\prime_\varplayer,\vardecision_{-\varplayer}) \!-\! \bar{\varcost}_\varplayer(\vardecision_\varplayer,\vardecision_{-\varplayer}) \!=\! \varpotentialfunction(\vardecision{}^\prime_\varplayer,\vardecision_{-\varplayer}) \!-\! \varpotentialfunction(\vardecision_\varplayer,\vardecision_{-\varplayer}). 
\end{equation}
\end{definition}

Next, let us recall a result from~\cite{harks2011characterizing} concerning the existence of an exact potential function in resource dependent congestion games.

\begin{lemma}~\cite{harks2011characterizing}\label{lem::potential_game_recall_result}
 Let $\varthegame = <\varactiveplayersset,(\varactivedecisionsset_\varplayer)_{\varplayer \in \varactiveplayersset},(\Tilde{\varcost}_\varplayer)_{\varplayer \in \varactiveplayersset}>$ be a weighted congestion game with resource-dependent weights in which the players compete over a finite set $\varresourcesset$ of resources.
 Then, the game $\varthegame$ has an exact potential function $\varpotentialfunction(\vardecisionsvector)$ if and only if the cost $\varresourcecost_\varresource(\vardecisionsvector)$ of sharing every resource $\varresource \in \varresourcesset$ is an affine function of the congestion on resource $\varresource$, i.e, $\varresourcecost_\varresource (\vardecisionsvector) = m_\varresource \varcongestionweight_\varresource(\vardecisionsvector) + n_\varresource$, $m_\varresource,n_\varresource \in \mathbb{R}$.
 The potential function $\varpotentialfunction(\vardecisionsvector)$ is given by 
 \begin{equation}\label{eq::potential_function_recall}
 \varpotentialfunction(\vardecisionsvector) = \sum \nolimits_{\varplayer \in \varactiveplayersset} \sum \nolimits_{\varresource \in \varresourcesset_{\vardecision_\varplayer}}\varcongestionweight_{\varplayer,\varresource}\varresourcecost_\varresource^{\leq \varplayer}(\vardecisionsvector),
 \end{equation}
 where $\varresourcecost_\varresource^{\leq \varplayer}(\vardecisionsvector) \!=\! m_\varresource \varcongestionweight_{\varresource}^{\leq \varplayer}(\vardecisionsvector) \!+\! n_\varresource$ and $\varcongestionweight_{\varresource}^{\leq \varplayer}(\vardecisionsvector) \!=\! \sum \limits_{\varoplayer \in \{\varoffloaders_\varresource(\vardecisionsvector)| \varoplayer \leq \varplayer\}}\!\!\!\!\!\!\!\!\varcongestionweight_{\varoplayer,\varresource}$.
 \end{lemma}
We can now formulate the following result on the existence of equilibria in the \ac{SL-COG}.
\begin{theorem}\label{theo::eq_potential_function_MS_COG}
The game $\varthegame(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^{\varslice,*},\varpolicy_\varcomppowercoef^{\varslice,*})$ has an exact potential function
 \begin{eqnarray}\label{eq::potential_function_MS_COG}
&\varpotentialfunction(\vardecisionsvector,\varpolicy_\varbandwidthcoef) = \sum_{\varplayer \in \varactiveplayersset} \sum_{\varresource \in \varresourcesset_{\vardecision_\varplayer} \cap \{\varAPsset  \times \varslicesset\}}\varcongestionweight_{\varplayer,\varresource}\varresourcecost_\varresource^{\leq \varplayer}(\vardecisionsvector,\varpolicy_\varbandwidthcoef) \nonumber\\
&+\sum_{\varplayer \in \varactiveplayersset} \sum_{\varresource \in \varresourcesset_{\vardecision_\varplayer} \cap \{\{\varcloudsset  \times \varslicesset\} \cup \varactiveplayersset\}}\varcongestionweight_{\varplayer,\varresource}\varresourcecost_\varresource^{\leq \varplayer}(\vardecisionsvector).
 \end{eqnarray}
\end{theorem}
\begin{proof}
The costs $\varresourcecost_{(\varAP,\varslice)}(\vardecisionsvector,\varpolicy_\varbandwidthcoef)$, $\varresourcecost_{(\varcloud,\varslice)}(\vardecisionsvector)$ and $\varresourcecost_{\varplayer}(\vardecisionsvector)$ are linear functions of $\varcongestionweight_{(\varAP,\varslice)}(\vardecisionsvector)$, $\varcongestionweight_{(\varcloud,\varslice)}(\vardecisionsvector)$ and $\varcongestionweight_{\varplayer}(\vardecisionsvector)$, respectively. Hence, Lemma~\ref{lem::potential_game_recall_result} applies, which proves the theorem.  
\end{proof}
\begin{comment}
\begin{proof}
Observe that the cost $\varresourcecost_{(\varAP,\varslice)}(\vardecisionsvector,\varpolicy_\varbandwidthcoef)$ is a linear function of the congestion $\varcongestionweight_{(\varAP,\varslice)}(\vardecisionsvector)$ on communication resource $(\varAP,\varslice)$ with $m_{(\varAP,\varslice)} = 1/\varbandwidthcoef_\varAP^\varslice$, the cost $\varresourcecost_{(\varcloud,\varslice)}(\vardecisionsvector)$ is a linear function of the congestion $\varcongestionweight_{(\varcloud,\varslice)}(\vardecisionsvector)$ on cloud computing resource $(\varcloud,\varslice)$ with $m_{(\varcloud,\varslice)} = 1/\varcomppower_\varcloud^\varslice$, and $\varresourcecost_{\varplayer}(\vardecisionsvector)$ is a linear function of the congestion $\varcongestionweight_{\varplayer}(\vardecisionsvector)$ on local computing resource $\varplayer$ with $m_{\varplayer} = 1/\varcomppower_\varplayer^\varlocal$. Hence, Lemma~\ref{lem::potential_game_recall_result} applies, which proves the theorem.  
\end{proof}
\end{comment}
Theorem~\ref{theo::eq_potential_function_MS_COG} allows us to formulate the following result.
\begin{corollary}\label{corr::SPE_existence_in_SL_COG}
The game $\varthegame(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^{\varslice,*},\varpolicy_\varcomppowercoef^{\varslice,*})$ has a pure strategy NE $\vardecisionsvector^*$. Thus for any $\varpolicy_\varbandwidthcoef$ the strategy profile  $(\vardecisionsvector^*,\varpolicy_\varbandwidthcoef, \varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$ is an SPE of the \ac{SL-COG}.
\end{corollary}
 \begin{proof}
 The existence of an exact potential function implies the existence of a pure strategy NE of the game $\varthegame(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^{\varslice,*},\varpolicy_\varcomppowercoef^{\varslice,*})$~\cite{monderer1996potential} and together with Corollary~\ref{cor::BR_of_slices_in_SL-COG} it implies the existence of an SPE of the \ac{SL-COG}.
 \end{proof}

So far we analyzed the interaction between WDs under the collection $(\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$ of equilibrium allocation policies of slices and an arbitrary allocation policy $\varpolicy_\varbandwidthcoef$ of the operator. In what follows we express the offloading cost of WD $\varplayer$ in the case when the operator uses policy $\varpolicy_\varbandwidthcoef^*$, which sets coefficients $\varbandwidthslicecoef_{\varAP}^{\varslice,*}$ according to (\ref{eq::optimal_operator_slice_coef}). 

\begin{corollary}\label{cor::congestion_game_device_cost_opt_operator}
Consider that the operator uses the equilibrium \rev{inter-slice radio} allocation policy $\varpolicy_{\varbandwidthcoef}^{*}$, which sets \rev{inter-slice radio} provisioning coefficients $\varbandwidthslicecoef_\varAP^{\varslice,*}$ according to (\ref{eq::optimal_operator_slice_coef}). Then, in the resulting strategic game $\varthegame(\varpolicy_\varbandwidthcoef^*,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$,the transmission cost of WD $\varplayer$ is independent on the chosen slice $\varslice$ and its cost is given by
%\vspace{-0.1cm}
\begin{equation}\label{eq::congestion_game_device_cost_opt_operator}
    \Bar{\varcost}_{\varplayer}(\vardecisionsvector) = \sum \nolimits_{\varresource \in \Bar{\varresourcesset}_{\vardecision_\varplayer}} \varcongestionweight_{\varplayer,\varresource}\varresourcecost_\varresource(\vardecisionsvector),
\end{equation}
where $\Bar{\varresourcesset}_{\vardecision_\varplayer} \subset \{\varAPsset \cup \{\varcloudsset \times \varslicesset\} \cup \{\varplayer\}\}$ and $\varresourcecost_{\varAP}(\vardecisionsvector)  = \varcongestionweight_{\varAP}(\vardecisionsvector) = \sum_{\varoplayer \in \varoffloaders_{\varAP}(\vardecisionsvector)}\sqrt{\vardatasize_\varoplayer/\varphywirelessrate_{\varoplayer,\varAP}}$.
\end{corollary}
\begin{proof}
From (\ref{eq::optimal_operator_slice_coef}) and (\ref{eq::AP_s_cost}) it follows that $\varresourcecost_{(\varAP,\varslice)}(\vardecisionsvector,\varpolicy_\varbandwidthcoef^*) \!\!=\!\! \sum \nolimits_{\varoslice \in \varslicesset} \varcongestionweight_{(\varAP,\varoslice)}(\vardecisionsvector)$. By defining the total congestion on AP $\varAP$ in strategy profile $\vardecisionsvector$ as $\varcongestionweight_\varAP(\vardecisionsvector) \triangleq \sum \nolimits_{\varoslice \in \varslicesset} \varcongestionweight_{(\varAP,\varoslice)}(\vardecisionsvector)$, we obtain that the cost of sharing AP $\varAP$ in strategy profile $\vardecisionsvector$ under the collection $(\varpolicy_\varbandwidthcoef^*,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$ of equilibrium policies of the operator and slices can be expressed as $\varresourcecost_\varAP(\vardecisionsvector) \!=\! \varcongestionweight_\varAP(\vardecisionsvector)$. Hence, we can express the cost (\ref{eq::congestion_game_device_cost}) of WD $\varplayer$ in game $\varthegame(\varpolicy_\varbandwidthcoef^*,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$ as (\ref{eq::congestion_game_device_cost_opt_operator}),
which proves the result.
\end{proof}
\begin{corollary}\label{theo::potential_function_MS_COG_opt_operator}
The exact potential function of the game $\varthegame(\varpolicy_\varbandwidthcoef^*,\varpolicy_\varuplinkratecoef^{\varslice,*},\varpolicy_\varcomppowercoef^{\varslice,*})$ is given by~(\ref{eq::potential_function_recall}).
\end{corollary}
\begin{proof}
Since $\varresourcecost_{\varAP}(\vardecisionsvector) \!=\! \varcongestionweight_{\varAP}(\vardecisionsvector)$, we can express the potential function (\ref{eq::potential_function_MS_COG}) as~(\ref{eq::potential_function_recall}), which proves the result.
\end{proof}
 From Corollary~\ref{corr::SPE_existence_in_SL_COG} and Theorem~\ref{theo::opt_sharing_policy_operator} we obtain the following result.
\begin{corollary}\label{corr::SPE_of_ES_COG}
The \ac{ES-COG} has an SPE $(\vardecisionsvector^*,\varpolicy_\varbandwidthslicecoef^*,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$.
\end{corollary}
In what follows we propose the \ac{COS} algorithm for computing a pure NE of the game $\varthegame(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$. The algorithm starts from an offloading strategy profile in which all WDs perform the computation locally and it allows them to update their BRs asynchronously. We show the pseudo code of the algorithm in Fig.~\ref{fig::COS}.

\begin{theorem}\label{theo::myopic_BR_algorithm}
 Consider the strategic game $\varthegame(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$ played by WDs for any feasible policy $\varpolicy_\varbandwidthcoef$ of the operator. An equilibrium $\vardecisionsvector{}^{*}$ of offloading decisions of WDs can be reached eventually by letting WDs to update their BRs according to the \ac{COS} algorithm.
\end{theorem}
\begin{proof}
The existence of an exact potential function implies that a pure NE of the game $\varthegame(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$ can be reached for any $\varpolicy_\varbandwidthcoef$ by letting WDs update their BRs asynchronously starting from an arbitrary strategy profile~\cite{monderer1996potential}.
\end{proof}

\begin{figure}[t]
	{\ruleline{$\vardecisionsvector{}^{*} = \ac{COS}(\varpolicy_\varbandwidthcoef,\varpolicy_\varuplinkratecoef^*,\varpolicy_\varcomppowercoef^*)$}
	 \vspace{-0.9cm}
	\begin{algorithm}[H]
		\While{\!$\exists$\!\! WD \!$\varoplayer \!\in\! \varactiveplayersset$ s.t. $\vardecision_\varoplayer \neq \argmin_{\vardecision{}^{\prime}_\varoplayer \in \varactivedecisionsset_\varoplayer}\! \Tilde{\varcost}_\varoplayer(\vardecision{}^{\prime}_\varoplayer,\! \vardecision_{-\varoplayer})$}
		 {
		 $\vardecision{}^{*}_\varoplayer=\argmin_{\vardecision{}^{\prime}_\varoplayer \in \varactivedecisionsset_\varoplayer} \Tilde{\varcost}_\varoplayer(\vardecision{}^{\prime}_\varoplayer, \vardecision_{-\varoplayer})$,
		 $\vardecisionsvector = (\vardecision{}^{*}_\varoplayer, \vardecision_{-\varoplayer})$
 	    }
 	    $\vardecisionsvector{}^{*} = \vardecisionsvector$
	\end{algorithm}
	\vspace{-0.4cm}
	\hrule
	\caption{Pseudo code of the \ac{COS} algorithm.}\label{fig::COS}
	\vspace{-0.6cm}}
\end{figure}
\subsection{Proposed Solution Implementation}
\label{subsec::implementation}

In what follows we discuss how an SPE of the \ac{ES-COG} can be implemented in practice. Given the information about the resource allocation policies of the operator and the slices, WDs perform BRs one at a time according to the \ac{COS} algorithm. Upon its turn, a WD computes the set of its BRs based on the information about
the congestion on the resources, as provided by the operator that acts as a coordinating entity. If the WD can improve its current offloading strategy then it reports one of its BRs to the operator, otherwise it reports its current offloading strategy. Since the operator is the leader in the \ac{NL-BAG}, it has information about the allocation policies of the slices, and thus by taking into account this information and the reported BR of the WD, it can recalculate the congestion on the resources and send the updated information to the next WD that is supposed to update its offloading decision. Upon convergence, given the equilibrium offloading decisions of WDs, the operator allocates bandwidth resources to slices according to policy $\varpolicy_\varbandwidthcoef^*$. Then, it informs the slices about the \rev{inter-slice radio} provisioning coefficients and the offloading decisions of the WDs, which use their own policies $\varpolicy_\varuplinkratecoef^{\varslice,*}$ and $\varpolicy_\varcomppowercoef^{\varslice,*}$ for allocating the bandwidth and the cloud computing resources to WDs. By Corollary~\ref{corr::SPE_of_ES_COG} the resulting state is an SPE of the \ac{ES-COG}.




==> solution_implementation.tex <==
\subsection{Proposed Solution Implementation}
\label{subsec::implementation}

In what follows we discuss how an SPE of the \ac{ES-COG} can be implemented in practice. Given the information about the resource allocation policies of the operator and the slices, WDs perform BRs one at a time according to the \ac{COS} algorithm. Upon its turn, a WD computes the set of its BRs based on the information about
the congestion on the resources, as provided by the operator that acts as a coordinating entity. If the WD can improve its current offloading strategy then it reports one of its BRs to the operator, otherwise it reports its current offloading strategy. Since the operator is the leader in the \ac{NL-BAG}, it has information about the allocation policies of the slices, and thus by taking into account this information and the reported BR of the WD, it can recalculate the congestion on the resources and send the updated information to the next WD that is supposed to update its offloading decision. Upon convergence, given the equilibrium offloading decisions of WDs, the operator allocates bandwidth resources to slices according to policy $\varpolicy_\varbandwidthcoef^*$. Then, it informs the slices about the \rev{inter-slice radio} provisioning coefficients and the offloading decisions of the WDs, which use their own policies $\varpolicy_\varuplinkratecoef^{\varslice,*}$ and $\varpolicy_\varcomppowercoef^{\varslice,*}$ for allocating the bandwidth and the cloud computing resources to WDs. By Corollary~\ref{corr::SPE_of_ES_COG} the resulting state is an SPE of the \ac{ES-COG}.
